AVeriTeC: A Dataset for Real-world Claim Verification with Evidence from the Web

Existing datasets for automated fact-checking have substantial limitations, such as relying on artificial claims, lacking annotations for evidence and intermediate reasoning, or including evidence published after the claim. In this paper we introduce AVeriTeC, a new dataset of 4,568 real-world claims covering fact-checks by 50 different organizations. Each claim is annotated with question-answer pairs supported by evidence available online, as well as textual justifications explaining how the evidence combines to produce a verdict. Through a multi-round annotation process, we avoid common pitfalls including context dependence, evidence insufficiency, and temporal leakage, and reach a substantial inter-annotator agreement of $\kappa=0.619$ on verdicts. We develop a baseline as well as an evaluation scheme for verifying claims through several question-answering steps against the open web.

==> sections/checklist.tex <==
\paragraph{Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?} Yes. Our primary contribution is the introduction of a high-quality dataset that avoids several common pitfalls. We rely on blind verification by human annotators to establish quality, as discussed in Section~\ref{section:annotation_process}.

\paragraph{Have you read the ethics review guidelines and ensured that your paper conforms to them?} Yes. We write substantially on the limitations and ethics of our paper in Sections~\ref{section:limitations} and~\ref{section:ethics}. With regards to wages for annotators, we worked with a company guaranteeing fair pay; see Section~\ref{appendix:appen}.

\paragraph{Did you discuss any potential negative societal impacts of your work?} Yes. We discuss in Section~\ref{section:ethics} how models trained on \datasetname could cause epistemic harm if applied for truth-telling, e.g. as automated content moderation systems. We have taken efforts to emphasize that neither our dataset nor models trained on it should be used as authoritative sources. As credibility is an important component in the effectiveness of fact-checking~\citep{berinsky_rumors_2017}, emphasizing that models trained on this dataset may not be credible can mitigate this potential harm.

\paragraph{Did you describe the limitations of your work?} Yes. We discuss limitations in Section~\ref{section:limitations}.

\paragraph{Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?} Yes. The code for our baseline can be found, along with our dataset, at \url{https://github.com/MichSchli/AVeriTeC}. We note that as the baseline relies on the Google Search API, it is not free; one run costs approximately £150. We can provide access to our cached search queries if requested by the reviewers.

\paragraph{Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?} Yes, see Section~\ref{section:baseline} and Appendix~\ref{appendix:baseline_prompts}.

\paragraph{Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?} No. As our baseline relies on the Google Search API, it is not free; one run costs approximately £150. Further, due to the restriction to 10.000 queries per day, one run can take up to three days. As such, the results we report in Section~\ref{section:experiments} are for one run only.

\paragraph{Did you include the amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?} Yes. See Section~\ref{section:baseline}, and Appendix~\ref{appendix:baseline_prompts} for further details.

\paragraph{If your work uses existing assets, did you cite the creators?} Yes. We mention the sources of our claims in Section~\ref{section:introduction}, and go into further details in Appendix~\ref{appendix:extra_statistics}. The models we use in our baseline are discussed and cited in Sections~\ref{section:baseline} and~\ref{section:experiments}.

\paragraph{Did you mention the license of the assets?} Yes, we mention in Section ~\ref{section:introduction} how all claims published through the Google FactCheck Claim Search API are available under a \textsc{CC-BY-4.0} license.

\paragraph{Did you include any new assets either in the supplemental material or as a URL?} Yes. The primary contribution of this paper is a new dataset, available at \url{https://github.com/MichSchli/AVeriTeC}.

\paragraph{Did you discuss whether and how consent was obtained from people whose data you're using/curating?} Yes. For the annotators, our instructions made it clear that the intention was to build a publicly available dataset; see Appendix~\ref{appendix:annotation_guidelines}. The claims in our dataset are based on publicly available from many different journalistic publications. As we mention in Section~\ref{section:ethics} we did not contact these, but we will remove claims originating from any journalist who requests it.

\paragraph{Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?} Yes. We discuss this in Section~\ref{section:ethics}.

\paragraph{Did you include the full text of instructions given to participants and screenshots, if applicable?}
Yes. The full instructions can be seen in Appendix~\ref{appendix:annotation_guidelines}.

\paragraph{Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?} No. We did not anticipate any risk for the participants, so we did not apply for an IRB. The claims we show to our annotators are screened by journalists in the context of fact-checking, so the chance of offensive context (beyond what might be seen on any news website) is low. Each participant had to go through a pilot phase before committing to working on the task, in order to build an understanding of what the task might require.

\paragraph{Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?} No. We worked with the crowdsourcing platform \textit{Appen}, who for annoymisation purposes could not provide us with the geographical location of each crowdworker. Appen pays a different rate (guaranteed at or above the local minimum wage) depending on location\footnote{https://success.appen.com/hc/en-us/articles/9557008940941-Guide-to-Fair-Pay}. As such, we cannot provide hourly wages per participant. The total amount spent on annotation, €40,835, can be found in Appendix~\ref{appendix:appen}.
